Unsupervised Crowdsourcing with Accuracy and Cost Guarantees

We consider the problem of cost-optimal utilization of a crowdsourcing platform for binary, unsupervised classification of a collection of items, given a prescribed error threshold. Workers on the crowdsourcing platform are assumed to be divided into multiple classes, based on their skill, experience, and/or past performance. We model each worker class via an unknown confusion matrix, and a (known) price to be paid per label prediction. For this setting, we propose algorithms for acquiring label predictions from workers, and for inferring the true labels of items. We prove that if the number of (unlabeled) items available is large enough, our algorithms satisfy the prescribed error thresholds, incurring a cost that is near-optimal. Finally, we validate our algorithms, and some heuristics inspired by them, through an extensive case study.

==> proof_sketches.tex <==
%%THEOREM 3.1
\begin{proofsketch}
Running steps (1)-(2) of \textit{Algorithm 2} of \citet{jordan} with $N$ items, returns the estimates $\{\hat{c}_k\}^M_{k=1}$. Parameterizing \begin{equation*}
    \epsilon=\frac{18}{\kappa^3_3 N^{\gamma}} \text{, and } \delta=M^2\exp\left(-\frac{N^{1-2\gamma} }{2}\right),
\end{equation*} 
it can be shown that for $N\geq \left( \frac{18}{ \bar{\kappa} \kappa^3_3 } \right)^{1/\gamma},$ 
    \begin{equation*}
       \max_{k \in [M]}\{ \|\hat{c}_k - c_k\| \} \leq \epsilon~ \textit{ w.p } \geq  1- \delta.
    \end{equation*}
To prove the bound on $\prob{\hat{k}\neq k^*}$, observe that \begin{align*}
        &\prob{\hat{k} \neq k^*} \\
        &= \prob{\bigcup_{k \in [M] \setminus k^*  }  \frac{p_{k^*}}{d(\hat{c}_{k^*},0.5)}  >  \frac{p_{k}}{d( \hat{c}_{k},0.5)} } \\
&\leq \begin{multlined} \prob{  \bigcup_{k \in [M] \setminus k^*   }  \frac{p_{k^*}}{d(c_{k^*} - \epsilon,0.5 )} > \frac{p_k}{d( c_k + \epsilon,0.5)} }  + \delta \end{multlined}\\
         &= \prob{ \begin{multlined}[c] \bigcup_{k \in [M] \setminus k^*   }  \frac{p_{k^*}}{d(c_{k^*} - \epsilon,0.5 )} - \frac{p_{k^*}}{d(c_{k^*},0.5)} \\ > \frac{p_k}{d(c_k+\epsilon,0.5)} -\frac{p_{k}}{d(c_{k},0.5)} + \Delta_k \end{multlined}} + \delta \numberthis \label{eq:khat}
    \end{align*}

For small enough~$\epsilon,$ the first term in~\eqref{eq:khat} is zero, yielding the desired bound on the probability of mis-identifying the optimal worker class. Specifically, the bounds $N \geq K_2$ and $N \geq K_3$ ensure that 
%
%The error in estimation, $\epsilon,$ decreases as $N$ becomes large, and so if $\epsilon$ can be kept below a certain threshold, the following bound on $\hat{c}_k$ 
%\begin{equation*}
%    c_k - \epsilon \leq \hat{c}_k \leq c_k + %\epsilon
%\end{equation*}
%is tight enough that the event in~\eqref{eq:khat} will be impossible. Specifically we want to ensure that
\begin{itemize}
    \item $\frac{p_{k^*}}{d(c_{k^*}-\epsilon,0.5 )} - \frac{p_{k^*}}{d(c_{k^*},0.5)} \leq \Delta_{min}/2 \leq \Delta_k/2,$
    \item  $\frac{p_{k}}{d(c_{k},0.5 )} - \frac{p_{k}}{d(c_{k} + \epsilon,0.5)} \leq \Delta_{k}/2$  $\forall k \in [M]\setminus k^*,$
\end{itemize}
which ensures that the first term in \eqref{eq:khat} is zero. The above claim is formalized by noting that $d(x, 0.5) = \log2 - H(x),$ where $H(\cdot)$ denotes the binary entropy function, and using following bounds:
%The additional lower bounds on $N$ combined with the fact that $d(x, 0.5) = \log2 - H(x)$ and the below inequalities on the binary entropy function
\begin{equation*}
    \frac{x}{2\log(\frac{6}{x})} \leq H^{-1}(x) \leq \frac{x}{\log(\frac{1}{x})}
\end{equation*}
The details can be found in Appendix~\ref{sec:appendix1}.

Finally, the claims about the accuracy of the final label assignment and the query-optimality follow from Lemma~\ref{thm:dtest}.

%help us prove that the above event in~\eqref{eq:khat} is indeed impossible.
\hide{
Within the event that all estimates are bounded within $\epsilon$, any worker class can be used in the exploit phase to assign labels with $\geq 1-\alpha$ accuracy. With a large enough $N$ and a small enough   $\epsilon$, we ensure that $\hat{c}_{k^*}$ remain close to its true value $c_{k^*}$ and consequently $\hat{k}=k^*$.Specifically, we use the following bounds on the binary entropy function.
\begin{equation*}
    \frac{x}{2\log(\frac{6}{x})} \leq H^{-1}(x) \leq \frac{x}{\log(\frac{1}{x})}
\end{equation*}
This combined with the additional bounds on $N$, ensure that \begin{itemize}
    \item $\frac{p_{k^*}}{d(c_{k^*}-\epsilon,0.5 )} - \frac{p_{k^*}}{d(c_{k^*},0.5)} \leq \Delta_{min}/2$
    \item  $\frac{p_{k}}{d(c_{k},0.5 )} - \frac{p_{k}}{d(c_{k} + \epsilon,0.5)} \leq \Delta_{k}/2$  $\forall k \in [M]\setminus k^*$
\end{itemize}
Combining the above, it is simple to observe that the UCB of $p_{k^*}\hat{s_{k^*}}$ will be well separated from the LCB of other worker classes to ensure that $\hat{k}$ is chosen optimally.}
\end{proofsketch}

%%THEOREM 3.2
\begin{proofsketch}
The proof is similar to that of Theorem~\ref{thm:sym}. Running Algorithm~1 of \citet{jordan} with $N$ items and one label each from each of the M worker classes, we get the confusion matrix estimates that satisfy \begin{equation*}
 \max_{k \in [M]} \norm{\hat{C}_k - C_k}_{\infty} \leq \epsilon =  N^{-\gamma_b} 
 \end{equation*} 
 w.p $\geq 1 - (48+M)\exp\left(1-N^{\gamma_a}\right)$
 if $N$ is larger than certain thresholds (given by Theorem~3 of \citet{jordan}). The parameterization of $\epsilon$ and $\delta$ as \begin{equation*}
    \epsilon= N^{-\gamma_b} \text{, and } \delta=(48+M)\exp\left(1-N^{\gamma_a}\right)
\end{equation*}  in terms of the parameters $\gamma_a, \gamma_b$ enables us to control~$\epsilon$ with $N.$ 
%and represent the thresholds purely in terms of instance parameters. 
The final requirement on $N$, i.e., $$N \geq \left|\frac{c_k(0)-c_k(1)}{2} \right|^{-1/\gamma_b} \iff \epsilon \leq \left|\frac{c_k(0)-c_k(1)}{2} \right|$$ ensures that $m_k = \argmin\{\hat{c}_k(0),\hat{c}_k(1)\}$, and \begin{align*}
         \frac{p_k}{d(\hat{c}_k(m_k), 0.5)} = \max \left\{\frac{p_k}{d(\hat{c}_k(0), 0.5)}, \frac{p_k}{d(\hat{c}_k(1), 0.5)}\right\}.
     \end{align*}
Now that the estimates $\{\hat{c}_k(0), \hat{c}_k(1)\}$ are ordered identical to their true values $\forall k \in [M]$, we can proceed in a similar manner using $c_k(m_k)$ instead of $c_k$ as done in the proof of Theorem~\ref{thm:sym}. The details can be found in Appendix~\ref{sec:appendix2}.
\hide{
The lower bounds on $N$, ensure that \begin{itemize}
    \item $\frac{p_{k^*}}{d(c^m_{k^*}-\epsilon,0.5 )} - \frac{p_{k^*}}{d(c^m_{k^*},0.5)} \leq \Delta_{min}/2$
    \item  $\frac{p_{k}}{d(c^m_{k},0.5 )} - \frac{p_{k}}{d(c^m_{k} + \epsilon,0.5)} \leq \Delta_{k}/2$  $\forall k \in [M]\setminus k^*$
\end{itemize}
which combined with the good event that all confusion matrix estimates are bounded within $\epsilon$ of their true values, ensure that $\hat{k}=k^*$.} 
\end{proofsketch}
%% OTHER



\begin{lemma} \label{lemma:lipschitz}
For any scalar $\frac{1}{2} < Y< 1$, the function $\theta(x,y)$ defined as 
\begin{equation*}\theta(x,y) = \frac{\lf{y}{1-x}}{\lf{xy}{(1-x)(1-y)}} \end{equation*}
is Lipschitz on $[\frac{1}{2},Y] \times [\frac{1}{2},Y]$, with Lipschitz constant $ \frac{Y - \frac{1}{2}}{2Y(1-Y)\lf{Y}{1-Y}}$\\


\end{lemma}
\begin{proof}
    \begin{equation}
        \deriv{\theta}{y}(x,y) = \frac{(1-y) - \theta(x,y)}{y(1-y)\lf{xy}{(1-x)(1-y)}}
    \end{equation}
    \begin{equation}\label{eq:dtdydx}
        \deriv{}{x}\deriv{\theta}{y} (x,y) = \frac{2\theta(x,y) - (x-y+1)}{x(1-x)(1-y)\left(\lf{xy}{(1-x)(1-y)}\right)^2}
    \end{equation}
    Now, we will prove that $\theta(x,y) \geq \frac{x + 1-y}{2} =: m_{xy}$ if and only if $x\geq y$. For this observe that \begin{align*}
        &d\left(\frac{x + 1-y}{2},x\right) - d\left(\frac{x + 1-y}{2},1-y\right)\\ &= \frac{x+1-y}{2}\lf{1-y}{x} + \frac{y+1-x}{2}\lf{y}{1-x}  \\ 
        &= \frac{1}{2} \left( d(1-y,x) - d(1-x,y)  \right)\\
        &\geq 0 ~~\, \text{(for $x\geq y$ , by Lemma \ref{lemma:klineq})}
    \end{align*} 
    Therefore we have $d(m_{xy},x) \geq d(\theta(x,y),x) = d(\theta(x,y),1-y) \geq d(m_{xy},1-y)$ which implies $m_{xy} \leq \theta(x,y)$ if $x\geq y$. Applying to  Eq (\ref{eq:dtdydx}), we have \begin{equation*} \{x\geq y\} \iff \deriv{}{x}\deriv{\theta}{y} \geq 0\end{equation*} and hence \begin{equation}
        \deriv{\theta}{y}(x,y) \geq \deriv{\theta}{y}(y,y) = \frac{ \frac{1}{2} -y}{2y(1-y)\lf{y}{(1-y)}} 
    \end{equation} 
    Moving to the next part, by Lemma \ref{con:decfunc}, we have $\deriv[2]{\theta}{y} (y,y)$ is a decreasing function in $y$, and so we can claim
    \begin{equation*} 0 \geq \deriv{\theta}{y} (x,y) \geq \frac{\frac{1}{2} - Y}{2Y(1-Y)\lf{Y}{1-Y}}\end{equation*}
    for all $x,y \leq Y$. Or Equivalently,
    
    \begin{equation*}
    \lvert \frac{}{} \deriv{\theta}{y} (x,y) \rvert \leq \frac{Y - \frac{1}{2} }{2Y(1-Y)\lf{Y}{1-Y}}
    \end{equation*}
\end{proof}


\begin{corollary} \label{cor:shifteps}
$d(\theta + \epsilon_1, c_1 - \epsilon_2) \geq d(\theta, c_1 - (\epsilon_1+\epsilon_2))$ if $(\epsilon_1+\epsilon_2) \leq c_1 + \theta -1$
\end{corollary}
\begin{proof}
    Applying Lemma \ref{lemma:dkldq}, with $q:= c_1 - \epsilon_1 - \epsilon_2$ and $c:=q -\theta$ with $(\epsilon_1+\epsilon_2) \leq c_1 + \theta -1$ implying that $q\geq (1+c)/2$
\end{proof}

\begin{corollary} \label{cor:shifteps2}
$d(\theta - \epsilon_1, c_1 + \epsilon_2) \geq d(\theta, c_1 + (\epsilon_1+\epsilon_2))$ if $(\epsilon_1-\epsilon_2) \leq c_1 + \theta -1$
\end{corollary}
\begin{proof}
    Applying Lemma \ref{lemma:dkldq}, with $q:= c_1 + \epsilon_2$ and $c:=q -\theta$ with $(\epsilon_1-\epsilon_2) \leq c_1 + \theta -1$ implying that $q\geq (1+c)/2$
\end{proof}


\begin{lemma}\label{lemma:klineq}
For $p,q>\frac{1}{2}$, it holds that $d(1-q,p) \geq d(1-p,q)$ if $p\geq q$
\end{lemma}
\begin{proof}
    \begin{equation*}
        d(p,q) = p\lf{p}{q} + (1-p)\lf{1-p}{1-q}     
    \end{equation*}
    
    \begin{equation}\label{eq:dkldq}
        \deriv{d}{p}(p,q) = \lf{p}{1-p} + \lf{1-q}{q} 
    \end{equation}
    Now we will attempt to compute $d(a,b)$  and $d(b,a)$ and make a comparison.
    \begin{align*}
        & d(b,a) - d(a,a) =  \int^b_a \deriv{d(p,a)}{p}dp \\
         &= \begin{multlined}[t] (b-a)\lf{1-a}{a} +  \int^b_a\lf{p}{1-p}dp  \\ \text{(Use $q=a$ in Eq (\ref{eq:dkldq}))}  \end{multlined} \numberthis\label{eq:klba} \\ 
    \end{align*}
    \begin{align*}
        & d(a,b) - d(b,b) =  \int^a_b \deriv{d(p,b)}{p}dp  \\
         &= \begin{multlined}[t] (a-b)\lf{1-b}{b} + \int^a_b\lf{p}{1-p}dp \\ \text{(Use $q=b$ in Eq (\ref{eq:dkldq}))}  \end{multlined} \\
         &= (b-a)\lf{b}{1-b} - \int^b_a\lf{p}{1-p}dp \numberthis\label{eq:klab}
    \end{align*}
    Now, subtracting Eq(\ref{eq:klab})  from Eq(\ref{eq:klba}), we obtain 
    \begin{align*}
        &d(a,b) - d(b,a) \\ &= \begin{multlined}[t] (b-a) \left( \lf{b}{1-b} - \lf{1-a}{a}\right) \\ - 2\int^b_a\lf{p}{1-p}dp \end{multlined}\\ 
        &= \begin{multlined}[t]
         (b-a) \left( \lf{b}{1-b} + \lf{a}{1-a}\right) \\ - 2\int^b_a\lf{p}{1-p}dp \end{multlined}
    \end{align*}
    Now, using $f(x) = \lf{x}{1-x}$ and $F(x) = \int \lf{x}{1-x}dx =  \log(1-x) + x\lf{x}{1-x}$, we write the same as
    \begin{align*}
        g(a,b) &= d(a,b) - d(b,a) \\ &= (b-a)\left(f(b) +f(a)\right) - 2(F(b)-F(a)) \\
        &= 2(b-a)\left(\frac{f(b) +f(a)}{2} - \frac{F(b)-F(a)}{b-a}\right)
    \end{align*}
    \begin{claim}\label{claim:gab}
    For $a$ and $b$ such that $\{0\leq 1-b \leq a \leq \frac{1}{2}\leq 1-a \leq b \leq 1 \}$ it is true that $g(a,b) \geq 0$
    \end{claim}
    \begin{claimproof}
        Note that  $g(a,1-a) = 0$ and\begin{align*}
            \deriv{g}{b}(a,b) &= (b-a)f^{'}(b) + (f(b) + f(a)) - 2f(b) \\ 
            &= (b-a)f^{'}(b) + f(a) - f(b) \\ 
            &= (b-a)\left( f^{'}(b) - \frac{f(b)-f(a)}{b-a} \right) \numberthis\label{eq:dgdb}
        \end{align*}
    Now we need to show that $\deriv{g}{b}(a,b)\geq 0$  for $b\geq 1-a \geq \frac{1}{2}$. A few  points to note are - \begin{itemize}
    \setlength\itemsep{0pt}
        \item $f(x)$ is an increasing function and  $f(\frac{1}{2}) = 0$ 
        \item $f(a) \leq 0$ and $f(b) \geq 0$
        \item $f(x)$ is convex in the region $\frac{1}{2}\leq x\leq 1$
    \end{itemize}
    We complete the proof in 2 parts - \begin{itemize}
        \item Since $f(x)$ is convex in the region $\frac{1}{2}\leq x\leq 1$, we can say that the gradient at $x=b$ will be greater than the slope of the line joining the points $(\frac{1}{2},0)$ to $(b,f(b))$ . Call this line $L1$. In other words - 
        \begin{equation*} f^{'}(b) \geq \frac{f(b) - 0}{b - \frac{1}{2}}\end{equation*}
        \item Notice that $\frac{f(b)-f(a)}{b-a}$ is the slope of the line joining the point $(a,f(a))$ to $(b,f(b))$. This line is represented by\begin{align*}
            y(x) &=  \frac{f(b)-f(a)}{b-a} \left(x -b\right) + f(b) \\
            y\left(\frac{1}{2}\right) &= \frac{f(b)-f(a)}{b-a} \left(\frac{1}{2} -b\right) + f(b)\\
            &= \left( \frac{\frac{1}{2} - a}{b-a}\right)f(b) + \left( \frac{b - \frac{1}{2}}{b-a}\right)f(a) \\
            &\geq 0 = f\left(\frac{1}{2}\right)
        \end{align*}
        Hence, $\frac{f(b)-f(a)}{b-a}$ has to be less than the slope of the line $L1$. In other words \begin{equation*}   \frac{f(b) - 0}{b -\frac{1}{2}} \geq \frac{f(b)-f(a)}{b-a}\end{equation*}
    \end{itemize}
    Combining both the above points, we have that \begin{equation*} f^{'}(b) \geq \frac{f(b)-f(a)}{b-a} \end{equation*} for $b \geq 1-a \geq \frac{1}{2}$ which proves that $\deriv{g}{b}(a,b)\geq 0$ and hence the claim
    \end{claimproof}
    % $\blacksquare$
    \\Due to Claim \ref{claim:gab}, we can say for $\frac{1}{2}\leq 1-a \leq b \leq 1$, it holds that \begin{equation*}d(a,b) \geq d(b,a)\end{equation*}
    Changing the parameters as $ p := b$ and $q := 1-a$, which now satisfy the requirements $p \geq q \geq \frac{1}{2}$,  it is true that \begin{equation*} d(1-q,p) \geq d(p,1-q) = d(1-p,q)\end{equation*}
\end{proof}


\begin{lemma}\label{con:decfunc}
The function \begin{equation*}f(y) := \frac{ \frac{1}{2} -y}{2y(1-y)\lf{y}{(1-y)}}  \end{equation*} is decreasing in $y$ for $\frac{1}{2}\leq y \leq 1$
\end{lemma}
\begin{proof}
    Proven. 
    \begin{align*}
        f^{'}(y) &= \deriv{f}{y}(y) = \frac{y -\frac{1}{2} - (y^2 - y + \frac{1}{2})\lf{y}{1-y}}{2y^2(1-y)^2 (\lf{y}{1-y})^2}  \\
        f^{'}(\frac{1}{2}) &= 0\\
        \text{Let, } g(y) &= y -\frac{1}{2} - (y^2 - y + \frac{1}{2})\lf{y}{1-y} \\ 
        g'(y) &=  1 - \frac{1}{2}\left(\begin{multlined}[t] (4y-2)\lf{y}{1-y} \\+ \frac{(y^2 + (1-y)^2)}{y(1-y)}\end{multlined}\right) \\
        &\leq 0 ~~ \text{(Since $\frac{(y^2 + (1-y)^2)}{y(1-y)} \geq 2$)}\\
        \implies  f^{'}(y) &\leq 0 ~~   \text{for $\frac{1}{2}\leq y \leq 1$ }
    \end{align*}
\end{proof}



\begin{lemma} \label{lemma:dkldq}
For any constant $0<c <1 $, the KL divergence, $d(q-c, q) = (q-c)\log{\frac{q-c}{q}} + (1-q+c)\log{\frac{1-q+c}{1-q}}  $ is increasing in $q$ for $q\geq \frac{1+c}{2}$
\end{lemma}
\begin{proof}
Let $f(q) = d(q-c, q)$
\begin{align*}
    \deriv{f(q)}{q} &=\begin{multlined}[t](q-c) \frac{q}{q-c}\frac{c}{q^2} +  \lf{q-c}{q} \\ + (1-q+c)\frac{1-q}{1-q+c}\frac{c}{(1-q)^2} \\ - \lf{1-q+c}{1-q} \end{multlined}\\
    &= \lf{(q-c)(1-q)}{(1-q+c)q} + \frac{c}{q} + \frac{c}{1-q} \\ 
    &= \log{\frac{q-c}{q}} + \log{\frac{1-q}{1-q+c}} + \frac{c}{q(1-q)} \\
    &\geq \left( 1- \frac{q}{q-c} \right) + \left( 1- \frac{1-q+c}{1-q} \right) + \frac{c}{q(1-q)} \\
    &= \frac{-c}{(q-c)(1-q+c)} + \frac{c}{q(1-q)} \\
    & = c\left(\frac{1}{q(1-q)} - \frac{1}{(q-c)(1-q+c)}\right) \\
    &= c^2 \frac{q - (1-q+c)}{q(1-q)(q-c)(1-q+c)} \\
    &\geq 0 \, \,  \text{     (For $q\geq (c+1)/2 $)}
\end{align*}
\end{proof}




\begin{lemma}\label{lemma:asym_epsbound}
For any quantity, $0 \leq \theta \leq c_1 \leq 1$ and $W,\epsilon>0$, it holds that \begin{equation*} \left\{ \epsilon \leq \frac{c_1(1-c_1)(e^{U} - 1)}{c_1 - \theta}\right\} \implies \left\{d(\theta, c_1 - \epsilon) \geq W\right\} \end{equation*} where $U = d(\theta, c_1) - W$
\end{lemma}
\begin{proof}
    \begin{align*}
        &d(\theta,c_1) - d(\theta, c_1 - \epsilon) \\
        &= \theta  \lf{c_1 - \epsilon}{c_1} + (1-\theta)\lf{1 - c_1 + \epsilon}{1-c_1} \\ 
        &\leq \log\left( \theta\frac{c_1 - \epsilon}{c_1} + (1-\theta)\frac{1 - c_1 + \epsilon}{1-c_1} \right) ~~\text{(Jensen's Inequality)} \\
        &= \log\left(1 + \frac{\epsilon(c_1 - \theta)}{c_1(1-c_1)}\right)
    \end{align*}
     
To complete the proof we need an upper bound on $\epsilon$ such that \begin{equation*} \log\left(1 + \frac{\epsilon(c_1 - \theta)}{c_1(1-c_1)}\right) \leq d(\theta, c_1) - W = U\end{equation*}
and $\epsilon \leq \frac{c_1(1-c_1)(e^{U} - 1)}{c_1 - \theta} $ satisfies that requirement.
\end{proof}

